The Effectiveness of Supervised Machine Learning Algorithms in Predicting Software Refactoring

Refactoring is the process of changing the internal structure of software to improve its quality without modifying its external behavior. Empirical studies have repeatedly shown that refactoring has a positive impact on the understandability and maintainability of software systems. However, before carrying out refactoring activities, developers need to identify refactoring opportunities. Currently, refactoring opportunity identification heavily relies on developers' expertise and intuition. In this paper, we investigate the effectiveness of machine learning algorithms in predicting software refactorings. More specifically, we train six different machine learning algorithms (i.e., Logistic Regression, Naive Bayes, Support Vector Machine, Decision Trees, Random Forest, and Neural Network) with a dataset comprising over two million refactorings from 11,149 real-world projects from the Apache, F-Droid, and GitHub ecosystems. The resulting models predict 20 different refactorings at class, method, and variable-levels with an accuracy often higher than 90%. Our results show that (i) Random Forests are the best models for predicting software refactoring, (ii) process and ownership metrics seem to play a crucial role in the creation of better models, and (iii) models generalize well in different contexts.

==> Makefile <==
BASE_NAME = paper
INPUTS    = $(wildcard *.tex) *.bib

LATEX     = latex
PDFLATEX  = pdflatex
BIBTEX    = bibtex
MAKEINDEX = makeindex

pdf: $(BASE_NAME).pdf
ps: $(BASE_NAME).ps

$(BASE_NAME).pdf: $(BASE_NAME).tex $(INPUTS)
	$(PDFLATEX) $<
	$(BIBTEX) $(BASE_NAME) 
	$(PDFLATEX) $< 
	$(PDFLATEX) $<
	#gs -q -dNOPAUSE -dBATCH -dPDFSETTINGS=/prepress -sDEVICE=pdfwrite -sOutputFile=$(BASE_NAME)wfonts.pdf $(BASE_NAME).pdf

clean:
	rm -f $(BASE_NAME)*.ps $(BASE_NAME)*.dvi *.log \
	      *.aux *.blg *.toc *.brf *.ilg *.ind \
	      missfont.log $(BASE_NAME)*.bbl $(BASE_NAME)*.pdf $(BASE_NAME)*.out \
		  $(BASE_NAME)*.lof $(BASE_NAME)*.lot 


==> fig-training-pipeline.tex <==
\begin{algorithm}[t]
\For{dataset $d$ in datasets}{
    \For{refactoring $r$ in refactorings}{
        \State $yes\_instances \gets refactorings\_for(d, r)$
        
        \State $no\_instances \gets non\_refactorings\_for(d,r)$
        
        \State $df \gets merge(yes\_instances, no\_instances)
        
        \State $df \gets balance(df)$
        
        \State df \gets scale(df)$
        
        \For{algorithm $a$ in ML algorithms}{
            \State $best\_params \gets random\_search(a, df,n\_iter=100, cv=10)$
            
            \State $model \gets a(best\_params)$
            
            \State $results \gets cross\_validate(model, df, cv=10)$
        }
    }
}
\caption{The training pipeline.}
\label{fig:training-pipeline}
\end{algorithm}
